Improving LLM Reasoning through Scaling Inference Computation with Collaborative Verification

Despite significant advancements in the general capability of large language models (LLMs), they continue to struggle with consistent and accurate reasoning, especially in complex tasks such as mathematical and code reasoning. One key limitation is that LLMs are trained primarily on correct solutions, reducing their ability to detect and learn from errors, which hampers their ability to reliably verify and rank outputs. To address this, we scale up the inference-time computation by generating multiple reasoning paths and employing verifiers to assess and rank the generated outputs by correctness. To facilitate this, we introduce a comprehensive dataset consisting of correct and incorrect solutions for math and code tasks, generated by multiple LLMs. This diverse set of solutions enables verifiers to more effectively distinguish and rank correct answers from erroneous outputs. The training methods for building verifiers were selected based on an extensive comparison of existing approaches. Moreover, to leverage the unique strengths of different reasoning strategies, we propose a novel collaborative method integrating Chain-of-Thought (CoT) and Program-of-Thought (PoT) solutions for verification. CoT provides a clear, step-by-step reasoning process that enhances interpretability, while PoT, being executable, offers a precise and error-sensitive validation mechanism. By taking both of their strengths, our approach significantly improves the accuracy and reliability of reasoning verification. Our verifiers, Math-Rev and Code-Rev, demonstrate substantial performance gains to existing LLMs, achieving state-of-the-art results on benchmarks such as GSM8k and MATH and even outperforming GPT-4o with Qwen-72B-Instruct as the reasoner.

==> tables/baseline.tex <==
\begin{table}[t]
\small
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabularx}{0.95\textwidth}{lcccccccccc}
\toprule
& \makecell{Greedy} & \makecell{Voting} & Recall & \makecell{ORM} & DPO & SimPO \\
\midrule
\multicolumn{8}{l}{\textit{\textbf{GSM8k:}}} \\
\hspace{0.2em}LLaMA2-7B-GSM8k & 40.18 & 53.83 & 92.27 & 64.29 & 65.13  & \textbf{69.14} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 33.97\%} & \textcolor{OliveGreen}{↑ 129.64\%} & \textcolor{OliveGreen}{↑ 59.95\%} & \textcolor{OliveGreen}{↑ 62.08\%} & \textcolor{OliveGreen}{↑ 72.08\%} \\
 %& \textcolor{blue}{43.55\%} & \textcolor{blue}{58.34\%} & \textcolor{blue}{100\%} & \textcolor{blue}{69.66\%} & \textcolor{blue}{70.59\%} & \textcolor{blue}{74.93\%} \\
\midrule
\hspace{0.2em}Mistral-7B-GSM8k & 55.80 & 76.50 & 98.48 & 76.59 & 77.03 & \textbf{81.43} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 37.10\%} & \textcolor{OliveGreen}{↑ 76.49\%} & \textcolor{OliveGreen}{↑ 37.29\%} & \textcolor{OliveGreen}{↑ 38.05\%} & \textcolor{OliveGreen}{↑ 45.93\%} \\
% & \textcolor{blue}{56.66\%} & \textcolor{blue}{77.69\%} & \textcolor{blue}{100\%} & \textcolor{blue}{77.76\%} & \textcolor{blue}{78.22\%} & \textcolor{blue}{82.69\%} \\
\midrule
\hspace{0.2em}Gemma-7B-it & 52.77 & 57.62 & 85.52 & 64.22 & 69.52 & \textbf{71.72} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 9.19\%} & \textcolor{OliveGreen}{↑ 62.06\%} & \textcolor{OliveGreen}{↑ 21.77\%} & \textcolor{OliveGreen}{↑ 31.71\%} & \textcolor{OliveGreen}{↑ 35.91\%} \\
% & \textcolor{blue}{61.70\%} & \textcolor{blue}{67.38\%} & \textcolor{blue}{100\%} & \textcolor{blue}{75.09\%} & \textcolor{blue}{81.29\%} & \textcolor{blue}{83.86\%} \\
\midrule
\hspace{0.2em}InternLM2-Math-7B & 84.38 & 89.08 & 98.33 & 90.22 & 90.98 & \textbf{91.12} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 5.57\%} & \textcolor{OliveGreen}{↑ 16.53\%} & \textcolor{OliveGreen}{↑ 6.92\%} & \textcolor{OliveGreen}{↑ 7.82\%} & \textcolor{OliveGreen}{↑ 7.99\%} \\
% & \textcolor{blue}{85.81\%} & \textcolor{blue}{90.61\%} & \textcolor{blue}{100\%} & \textcolor{blue}{91.74\%} & \textcolor{blue}{92.53\%} & \textcolor{blue}{92.67\%} \\
\midrule
\hspace{0.2em}Phi3-14B & 86.73 & \textbf{93.56} & 99.24 & 92.80 & 92.26 & \textbf{93.56} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 7.88\%} & \textcolor{OliveGreen}{↑ 14.42\%} & \textcolor{OliveGreen}{↑ 7.00\%} & \textcolor{OliveGreen}{↑ 6.38\%} & \textcolor{OliveGreen}{↑ 7.88\%} \\
% & \textcolor{blue}{87.39\%} & \textcolor{blue}{94.28\%} & \textcolor{blue}{100\%} & \textcolor{blue}{93.51\%} & \textcolor{blue}{92.97\%} & \textcolor{blue}{94.28\%} \\
\midrule
\hspace{0.2em}LLaMA3-70B-instruct & 94.39 & 95.22 & 98.48 & 92.80 & 93.89 & \textbf{95.29} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 0.88\%} & \textcolor{OliveGreen}{↑ 4.33\%} & \textcolor{negative}{↓ 1.68\%} & \textcolor{negative}{↓ 0.53\%} & \textcolor{OliveGreen}{↑ 0.95\%} \\

\midrule
\multicolumn{7}{l}{\textit{\textbf{MATH500:}}} \\
\hspace{0.2em}LLaMA3-8B-Instruct & 30.00 & \textbf{36.80} & 69.80 & 31.20 & 31.80 & 33.40 \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 22.67\%} & \textcolor{OliveGreen}{↑ 132.67\%} & \textcolor{OliveGreen}{↑ 4.00\%} & \textcolor{OliveGreen}{↑ 6.00\%} & \textcolor{OliveGreen}{↑ 11.33\%} \\
 \midrule
\hspace{0.2em}Mistral-Instruct-v0.3 & 12.80  & 21.00 & 58.00 & 14.00 & 17.60 & \textbf{21.80} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 64.06\%} & \textcolor{OliveGreen}{↑ 353.12\%} & \textcolor{OliveGreen}{↑ 9.38\%} & \textcolor{OliveGreen}{↑ 37.50\%} & \textcolor{OliveGreen}{↑ 70.31\%} \\
 
 \midrule
\hspace{0.2em}Gemma-7B-it & 16.20 & 23.80 & 57.20 & 20.20 & 24.80 & \textbf{26.00} \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 46.91\%} & \textcolor{OliveGreen}{↑ 253.09\%} & \textcolor{OliveGreen}{↑ 24.69\%} & \textcolor{OliveGreen}{↑ 53.09\%} & \textcolor{OliveGreen}{↑ 60.49\%} \\

 \midrule
\hspace{0.2em}InternLM2-Math-7B & 35.80 & \textbf{55.80} & 77.80 & 45.40 & 48.00 & 51.20 \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 55.87\%} & \textcolor{OliveGreen}{↑ 117.32\%} & \textcolor{OliveGreen}{↑ 26.82\%} & \textcolor{OliveGreen}{↑ 34.08\%} & \textcolor{OliveGreen}{↑ 43.02\%} \\

 \midrule
\hspace{0.2em}Phi3-14B & 23.60 & \textbf{46.00} & 73.80 & 33.80 & 36.60 & 38.40 \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 94.92\%} & \textcolor{OliveGreen}{↑ 212.71\%} & \textcolor{OliveGreen}{↑ 43.22\%} & \textcolor{OliveGreen}{↑ 55.08\%} & \textcolor{OliveGreen}{↑ 62.71\%} \\

 \midrule
\hspace{0.2em}LLaMA3-70B-instruct & 50.40 & \textbf{59.20} & 87.00 & 48.20 & 49.00 & 51.80 \\
 & \textcolor{black}{0\%} & \textcolor{OliveGreen}{↑ 17.46\%} & \textcolor{OliveGreen}{↑ 72.62\%} & \textcolor{red}{↓ 4.37\%} & \textcolor{red}{↓ 2.78\%} & \textcolor{OliveGreen}{↑ 2.78\%} \\


        \bottomrule
    \end{tabularx}}
    \caption{Performance metrics for various models on GSM8k and MATH500 datasets, including Base Acc./Improvement/Ratio to Oracle (Recall)?}
    \label{tab:performance}
\end{table}

==> tables/qwen.tex <==
\begin{table}[h]
\small
    \centering
    \begin{tabularx}{0.93\textwidth}{lcccc}
        \toprule

        \textit{\textbf{Math Reasoning Leaderboard}} & Size & Open & GSM8k & MATH \\
        \midrule
        GPT-3.5-Turbo & ? & \xmark & 92.0 & 42.5 \\
        Gemini-1.5-Pro (May) \citep{reid2024gemini} & ? & \xmark & 90.8 & 67.7 \\
        Claude3-Opus & ? & \xmark & 95.0 & 60.1 \\
        GPT-4-1106 & ? & \xmark & 91.4 & 64.3 \\
        GPT-4-turbo & ? & \xmark & 94.7 & 73.4 \\
        GPT-4o & ? & \xmark & 95.8 & 76.6 \\
        LLaMA3-70B-SFT \citep{lai2024step} & 70B & \cmark & 88.2 & 54.8 \\
        Qwen-72B-Instruct \citep{yang2024qwen2} & 72B & \cmark & 92.4 & 69.4 \\
        DeepSeek-Coder-V2-Instruct \citep{zhu2024deepseek} & 236B & \cmark & 94.9 & 75.7 \\
        Gemini + OmegaPRM \citep{luo2024improve} & ? & \xmark & - & 72.4  \\
        Qwen2-72B-SFT + Step-DPO \citep{lai2024step} & 72B & \cmark & 94.0 & 70.8 \\
        NuminaMath 72B TIR \citep{numina_math_7b} & 72B & \cmark & 91.5 & 75.8\\
        %... & & & &\\
        %Our Verifier @ 64 & & \\
        LLaMA3.1-70B-Instruct & 70B & \cmark & 95.1 & 68.0 \\
        LLaMA3.1-405B-Instruct & 405B & \cmark & \textbf{96.8} & 73.8 \\
        Math-Rev \& Qwen-72B-Instruct (Ours)& 72B+7B & \cmark & 95.1 & \textbf{76.9} \\
        Math-Rev + CoTnPoT \& Qwen-72B-Instruct (Ours)& 72B+7B+16B & \cmark & 95.6 & 75.3 \\

        \bottomrule
    \end{tabularx}
    \caption{Placing our performance on the leaderboard.}
    \label{tab:mistral_results}
\end{table}
